A Hopfieldian View-based Interpretation for Chain-of-Thought Reasoning

Chain-of-Thought (CoT) holds a significant place in augmenting the reasoning performance for large language models (LLMs). While some studies focus on improving CoT accuracy through methods like retrieval enhancement, yet a rigorous explanation for why CoT achieves such success remains unclear. In this paper, we analyze CoT methods under two different settings by asking the following questions: (1) For zero-shot CoT, why does prompting the model with "let's think step by step" significantly impact its outputs? (2) For few-shot CoT, why does providing examples before questioning the model could substantially improve its reasoning ability? To answer these questions, we conduct a top-down explainable analysis from the Hopfieldian view and propose a Read-and-Control approach for controlling the accuracy of CoT. Through extensive experiments on seven datasets for three different tasks, we demonstrate that our framework can decipher the inner workings of CoT, provide reasoning error localization, and control to come up with the correct reasoning path.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> section/6_case_analysis.tex <==

\section{Case Analysis}

To further demonstrate the effectiveness of our approach, we provide three cases in three models on arithmetic, commonsense and symbolic reasoning tasks.

For zero-shot CoT, Figure~\ref{fig:case_aqua_zero} displays the real prediction of a case by the model both without control and control. 
From this figure, we can observe that the model is wrong when simplifying the equation, and the reasoning path is offset. 
As shown in the \textcolor{salmon}{red} part, the reason for the mistake of the model is that multiple steps have been performed in the process of simplification, which leads to calculation errors.
After adding control to the model, the direction of the reasoning path of the model will be corrected to achieve the calculation error that occurs when the control is not added.

For few-shots CoT, Figure~\ref{fig:case_strategyqa_few} demonstrates the real prediction of a case by the model both without control and with control on the strategyQA dataset.  From this figure, we can observe that the model initially makes a correct inference regarding the elevation of Mount Fuji and the depth of the Sea of Japan. However, the model erroneously concludes that Mount Fuji would not be out of the sea due to a miscalculation in comparing the mountain’s height with the sea’s depth as illustrated in the red segment.  After adding control to the model, the reasoning path leads to the correct conclusion that the top of Mount Fuji would indeed be out of the Sea of Japan, as highlighted in the green segment. Additionally, Figure~\ref{fig:few_shot_case_llama3_coin_flip} also showcases that the model initially makes a correct inference step by step about the coin's state after each flip.  However, the error arises from not correctly accounting for the even number of flips by Kydin. After adding control, the model correctly reasons that the coin has flipped a total of two times, an even number, leading to the accurate conclusion that the coin remains heads up, as shown in the \textcolor{salmon}{green} segment. These demonstrate the significance of control in ensuring the model follows the correct reasoning path.

==> tables/fig2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/LAT.pdf}
    \caption{The pipeline of LAT. \warn{unfinished DO WE NEED THIS FIGURE..?}}
    \label{fig:lat}
\end{figure}

==> tables/main_result.tex <==
% \begin{table*}[]
% \centering
% % \resizebox{}{!}{%
% \begin{tabular}{lcccccccc}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c}{Arithmetic Reasoning} & \multicolumn{3}{c}{Commonsense Reasoning} & \multicolumn{2}{c}{Symbolic Reasoning} \\ \cline{2-9} 
%  & GSM8K & SVAMP & AQuA  & StrategyQA & \begin{tabular}[c]{@{}c@{}}Date Under.\end{tabular} & \begin{tabular}[c]{@{}c@{}}CSQA\end{tabular} & Coin Flip & Random Letter \\ \hline
% \multicolumn{9}{c}{zero-shot CoT} \\ \hline
% Mistral-7B-instruct & / & / & / & 63.01 / & / & / & / & / \\
% LLaMA-2-7B-chat & 26.31 / \textbf{27.37} & \textbf{46.00} / 44.00 & 27.95 / \textbf{30.71} & 62.66 / \textbf{63.49} & / & 55.45 / \textbf{56.59} & 52.20 / \textbf{55.75} & / \\
% LLaMA-3-8B-instruct & 74.45 / \textbf{75.89} & / & / & 67.42 / \textbf{68.03} & / & / & \textbf{93.05} / 85.90 & / \\ \hline
% \multicolumn{9}{c}{few-shot CoT} \\ \hline
% Mistral-7B-instruct & / & 61.33 / \textbf{61.67} & 34.65 / \textbf{35.04} & 63.49 / \textbf{65.55} & / & / & / & / \\
% LLaMA-2-7B-chat & 5.00 / \textbf{5.16} & 38.67 / \textbf{39.00} & 22.44 / \textbf{23.62} & / & / & 55.61 / \textbf{58.56} & 49.47 / \textbf{49.84} & / \\
% LLaMA-3-8B-instruct & 72.71 / \textbf{74.83} & \textbf{82.00} / 81.67 & 52.76 / \textbf{53.21} & 60.39 / \textbf{69.13} & / & / & 77.02 / \textbf{77.59} & / \\ \hline
% \end{tabular}%
% % }
% \caption{The results of our method in different models, the left side is the score without control, and the right side is after control. \warn{The improving means this number is improving by parameter grid search so that it will be modified(just a note)} }
% \label{tab:main_result}
% \end{table*}



\begin{table*}[ht]
\centering
% \resizebox{0.95\textwidth}{!}{
\resizebox{\textwidth}{!}{
\begin{tabular}{lccccccc}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c}{Arithmetic Reasoning} & \multicolumn{2}{c}{Commonsense Reasoning} & \multicolumn{2}{c}{Symbolic Reasoning} \\ \cline{2-8} 
 & GSM8K & SVAMP & AQuA & StrategyQA & CSQA & Coin Flip & Random Letter \\ \hline
\multicolumn{8}{c}{zero-shot CoT} \\ \hline
Mistral-7B-instruct & 45.03 / \textbf{47.08} & 57.33 / \textbf{61.33} & 25.59 / \textbf{30.71} & 63.01 / \textbf{63.97} & 67.57 / \textbf{67.98} & \textbf{50.80} / 48.95 & / \\
LLaMA-2-7B-chat & 26.31 / \textbf{27.37} & 46.00 / \textbf{46.67} & 27.95 / \textbf{30.71} & 62.66 / \textbf{63.49} & 55.45 / \textbf{56.59} & 52.20 / \textbf{55.75} & \textbf{17.33} / 15.33 \\
LLaMA-3-8B-instruct & 74.45 / \textbf{75.89} & 82.67 / \textbf{84.00} & 42.13 / \textbf{45.67} & 67.42 / \textbf{68.03} & \textbf{45.29} / 44.39 & \textbf{90.45} / 88.90 & \textbf{38.00} / 37.33 \\ 
AVG. & 48.60 / 50.11 (\textbf{1.51↑}) & 62.00 / 64.00 (\textbf{2.00↑}) & 31.89 / 35.70 (\textbf{3.81↑})  &  64.36 / 65.16 (\textbf{0.80↑}) &  &  & / \\ \hline
\multicolumn{8}{c}{few-shot CoT} \\ \hline
Mistral-7B-instruct & 46.78 / \textbf{47.16} & 61.33 / \textbf{61.67} & 34.65 / \textbf{35.04} & 63.49 / \textbf{65.55} & 52.83 / \textbf{54.87} & \textbf{78.73} / 78.19 & 33.67 / 33.67 \\
LLaMA-2-7B-chat & 5.00 / \textbf{5.16} & 38.67 / \textbf{39.00} & 22.44 / \textbf{23.62} & 55.63 / \textbf{55.72} & 55.61 / \textbf{58.56} & 50.74 / \textbf{50.84} & 29.67 / \textbf{30.00} \\
LLaMA-3-8B-instruct & 72.71 / \textbf{74.83} & 82.00 / \textbf{83.67} & 52.76 / \textbf{53.21} & 66.38 / \textbf{68.47} & 67.24 / \textbf{68.47} & 77.02 / \textbf{77.59} & 53.67 / \textbf{54.67}  \\
AVG. & 41.50 / 42.38 (\textbf{0.88↑}) &  60.67 / 61.45 (\textbf{0.78↑}) & 36.61 / 37.29 (\textbf{0.68↑}) & 61.83 / 63.25 (\textbf{1.42↑}) & 58.56 / 60.63 (\textbf{2.07↑}) & 68.83 / 68.87 (\textbf{0.04↑}) & 39.00 / 39.45 (\textbf{0.45↑}) \\ \hline
\end{tabular}
}
\caption{The results of our method in different models, the left side is the score without control, and the right side is after control. The AVG. presented in the table denote the overall improvement for each task applying the control method.}
\label{tab:main_result}
\end{table*}


==> tables/nnrepresentation_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/nn_representation.pdf}
    \caption{nn\_rep~\warn{Todo change to mini page and write a new caption}}
    \label{fig:nnrep}
\end{figure}

==> tables/stimulus_figure.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\linewidth]{figures/stimulu.pdf}
    \caption{stimulu~\warn{Todo: change to mini page and write a new caption}}
    \label{fig:stimulu}
\end{figure}

==> tables/table_answer_cleansing.tex <==
\begin{table}[h]\centering
%\footnotesize
\caption{Detail description of answer cleansing. See \autoref{tab:dataset_description} for the mapping between each datasets and the corresponding answer formats.}
\label{tab:answer_cleansing}
\begin{tabular}{p{0.15\textwidth}p{0.25\textwidth}p{0.40\textwidth}}
%\begin{tabular}{lrrr}
\toprule
Answer \par Format &Answer Cleansing \par Approach &Pseudo Code \par (Example in Pytorch 3.8) \\\midrule \midrule
Number &Pick up the first number encountered in the text. &
\begin{lstlisting}
pred = pred.replace(",", "")
pred = [s for s in re.findall(r'-?\d+\.?\d*', pred)]
pred = pred[0] 
\end{lstlisting}

\\
\midrule

Multiple-Choice &Pick up the first large letter encountered in the text. &
\begin{lstlisting}
pred = re.findall(r'A|B|C|D|E', pred) 
pred = pred[0]
\end{lstlisting}

\\\midrule

Yes or No &Pick up the first "yes" or "no" encountered in the text after removing unnecessary letters. &
\begin{lstlisting}
pred = pred.lower()
pred = re.sub("\"|\'|\n|\.|\s|\:|\,"," ", pred) 
pred = pred.split(" ") 
pred = [i for i in pred if i in ("yes", "no")] 
pred = pred[0]
\end{lstlisting}

\\\midrule

Free Format &Just remove unnecessary letters, such as ".". &
\begin{lstlisting}
pred = re.sub("\"|\'|\n|\.|\s","", pred)
\end{lstlisting}

\\

\bottomrule
\end{tabular}
\end{table}
